A WSPD, Separator and Small Tree Cover for c-packed Graphs

The $c$-packedness property, proposed in 2010, is a geometric property that captures the spatial distribution of a set of edges. Despite the recent interest in $c$-packedness, its utility has so far been limited to Fr\'echet distance problems. An open problem is whether a wider variety of algorithmic and data structure problems can be solved efficiently under the $c$-packedness assumption, and more specifically, on $c$-packed graphs. In this paper, we prove two fundamental properties of $c$-packed graphs: that there exists a linear-size well-separated pair decomposition under the graph metric, and there exists a constant size balanced separator. We then apply these fundamental properties to obtain a small tree cover for the metric space and distance oracles under the shortest path metric. In particular, we obtain a tree cover of constant size, an exact distance oracle of near-linear size and an approximate distance oracle of linear size.

==> 8.1_GWSPD_Correctness.tex <==
%------------------------CORRECTNESS-------------------------

\subsection{Correctness}
\label{subsec:correctnessWSPD}
To prove the correctness of the WSPD$_G$ construction we first prove in Lemma~\ref{lem:valid_GST} that $T$ is a valid \GST{$c$}. We then prove in Lemma~\ref{lem:correctnessDiamUb} that the value \gdub{u}, computed as described in Section~\ref{subsec:upperbounddiam}, is a valid upper bound on the graph diameter of the connected subgraph represented in cell $u$, for all cells $u \in T$. We then prove in Lemma~\ref{lem:size_and_separation_WSPDG} that the pairs of the resulting WSPD$_G$ $W$ are $\sigma$-well separated and $W$ is of size $O(c^3 \sigma n)$.


\begin{lemma}
    \label{lem:valid_GST}
    Given a $c$-packed graph $G(V,E)$ the above algorithm produces a valid $c$-connected tree $T$ of $G(V,E)$.
\end{lemma}\lnote{Proof is fairly straightforward. Move to appendix?}
\begin{proof}
    To prove the lemma, it is clear from Definition~\ref{def:gst} that it only remains to prove that every node in $T$ is a $c$-connected set in $G$. That is, consider any node $u$ in $T$ and let $p$ and $q$ be any two points stored in the leaves of the subtree rooted at $u$. We will need to prove that $\gdist{p}{q} \leq c \cdot \diam{s(u)}$.
    
    Let $v(p)$ and $v(q)$ be the leaves storing $p$ and $q$ and let $v$ be the lowest common ancestor of $v(p)$ and $v(q)$ in $T$. Let $s(v)$ denote the cube corresponding to node $v$. We claim that the shortest path between $p$ and $q$ in $G$ must lie entirely within a cube $s^+(v)$ of diameter twice the diameter of $s(v)$, centered at $s(v)$. This follows from the fact that every cube and corresponding cube of twice the diameter on the path from $v(p)$ (resp. $v(q)$) to $v$ must lie strictly within $s^+(v)$. From the $c$-packedness of the original graph we deduce that the length of the path between $p$ and $q$ can be at most $2c\cdot \radius{s(v)} = c \cdot \diam{s(v)}$. 

    This allows us to conclude that, since $\diam{s(v)}$ is the smallest diameter of any cell in which $p$ and $q$ appear together, it holds for all cells of $T$ that the original graph distance between any two points contained in the leaves of its subtree, is at most $c$ times the diameter of the cell. We conclude that $T$ is indeed a valid \GST{$c$}.
\end{proof}

Next, we prove the value \gdub{u}, computed in Section~\ref{subsec:upperbounddiam} is a valid upper bound on the graph diameter of the connected subgraph represented in a cell of $T$. The proof of Lemma~\ref{lem:correctnessDiamUb} can be found in Section~\ref{sec:correctnessDiamUb} in the Appendix. 

\begin{restatable}{lemma}{correctnessDiamUb}
    \label{lem:correctnessDiamUb}
    The value \gdub{v} for any cell in $v \in T$ upper bounds the graph diameter of the connected subgraph represented in the cell $v$.
\end{restatable}

\begin{toappendix}
\section{Proofs for Section~\ref{sec:GWSPD} (A Well-Separated Pair Decomposition for $c$-packed Graphs)}
\subsection{Proof of Lemma~\ref{lem:correctnessDiamUb}} 
    \label{sec:correctnessDiamUb}
    \correctnessDiamUb*
\begin{proof}
    Let $u\in Q$ be the original cell in the compressed quadtree $Q$ that $v \in T$ was created from in Section~\ref{subsec:c_CT}. To argue \gdub{v} is a valid upper bound on the graph diameter of the connected component corresponding to cell $v \in T$ we argue that it correctly upper bounds the graph diameter of \emph{any} connected component contained in $u$\lnote{Would this be less confusing if instead we apply the lemma to any connected component in Q and then as a corollary apply it to any node in T?}. 
    Since the original connected component in $G$ contained in any cell $u \in Q$ is fully contained within a cube of twice the radius of $u$, centered at $u$, we conclude that the graph diameter of any connected component represented by $u$ is at most $\rel{s(u)} + \sum_{s \in N(s(u)}\rel{s}$\lnote{We already mention this in algorithm description. Perhaps only mention here or there, not both?}. It thus remains to argue that $\rel{s}$ for any canonical cube $s$ is correctly computed in Section~\ref{subsec:upperbounddiam}.

    We first argue that for all cells $w$ in $Q_S$, the value stored at the cell is equal to $\rel{s(w)}$. This follows from the fact that only edges of length at most twice the diameter contribute to this value. Since the canonical cells are the lowest cells in the compressed quadtree that overlap with relevant edges, it follows that the bottom-up summation of the values correctly maintains $\rel{s(w)}$ for all $w \in Q_S$.\lnote{Does this argument suffice?}

    Next, for all canonical cubes $s_c$ that have non-zero relative edge length, let $w$ be a node in $Q_S$ who's corresponding cube is the largest cube fully contained inside $s_c$. We argue $\rel{s(w)} = \rel{s_c}$.\lnote{This follows from either same size --> follows trivially. Otherwise, only non-empty child of parent. --> trivial.}
\end{proof}
\end{toappendix}
Next, to bound the size of the resulting WSPD$_G$ we introduce the following lemmas.
\begin{lemma}
 \label{lem:bounding_m_c-packed}
    Let $G(V,E)$ be a $c$-packed graph. For any cube $s$, there exists a $c$-connected partition $\CP{c}{V(s)}$ of size at most $O(c)$.\lnote{$O(c\sqrt{d})$}\lnote{This lemma can be moved to the appendix but that does not leave many proofs in this section.}
\end{lemma}
\begin{proof}
    Consider a cube $s$ of radius $r$ centered at a point $p$, and let $s^+$ be a cube with radius $2r$ centered at $p$. Partition $V(s)$ into maximal sets $\{C_1, \ldots ,C_k\}$ such that the vertices in a set $C_i$ are connected by a tree of $G$ that lies entirely within $s^+$. We will show (i) the length of the path between any two points in a set is at most $c\cdot \diam{s}$, and (ii) $k\leq 2c\sqrt{d} +1$.

    We prove (i) by observing that for any two points in $V(s)$ that have a path connecting them that lies entirely within $s^+$, the graph distance between the two points is at most $2rc = c\cdot \diam{s}$. This follows immediately from the fact that $G$ is $c$-packed. 
    
    To prove (ii), we note that in order for any pair of points in $V(s)$ to be disconnected within $s^+$, every path between them must intersect the boundary of $s^+$ and therefore have length at least $\frac{r}{\sqrt{d}}$, as shown in Figure~\ref{fig:nmbr_CC}. From the $c$-packedness of $G$ we conclude there cannot exist more than $\frac{2cr\sqrt{d}}{r} = 2c\sqrt{d}$ such paths in $s^+$, completing the proof of the lemma.
\end{proof}

\begin{figure}[H]
	\begin{center}
		\includegraphics[scale=0.15]{delta-connected_sets.png}
		\caption{Two $\delta$-connected components in $s$ must be separated by a path of length at least $\frac{\radius{s}}{\sqrt{d}}$.}
		\label{fig:nmbr_CC}
	\end{center}
\end{figure} 

Finally, to analyse the size of the resulting WSPD$_G$ we employ the help of the following two lemmas.
The proof of Lemmas~\ref{lem:rep_c_connect} and~\ref{lem:number_nodes_per_cell} can be found in Sections~\ref{sec:repcconnect} and~\ref{sec:nodespercell} in the Appendix.

\begin{restatable}{lemma}{repcconnected}
\label{lem:rep_c_connect}
    For all $u \in U_{i_j}$, $1\leq j \leq \ell$, each vertex in $H_{i_j}$ within $s(u)$ represents a $c$-connected component in $H_{i_{j-1}}$ with respect to the diameter of $s(u)$.
\end{restatable}

\begin{toappendix}
\subsection{Proof of Lemma~\ref{lem:rep_c_connect}}
\label{sec:repcconnect}
\repcconnected*
\begin{proof}
    We argue the algorithm maintains this property by induction on the number of iterations. The algorithm initially uses as input the $c$-packed graph $H_{i_1} = H_{i_0} = G$. After the first iteration of the algorithm, for each node $u \in U_{i_1}$, each surviving point $x$ in $V_{i_1}$ represents a set of points in $V_{i_0}$ that were connected to $x$ within $s^+(u)$. Since $H_{i_0} = G$ is $c$-packed, we can conclude that the distance between $x$ and any point merged into $x$ is at most $c$ times the radius of $s^+(u)$, and therefore $c$ times the diameter of $s(u)$. 
    
    Assume that the algorithm maintains the invariant for iterations 1 to $k < \ell$. Note that the graph $H_{i_k}$, used as input for iteration $k+1$, is no longer guaranteed to satisfy $c$-packedness. However, observe that after each merge step, the representative nodes in $V_{i_{k+1}}$ always correspond to original nodes present in $G$. Since the process of merging each connected set into a single node can only reduce the length of the paths between the remaining representatives, the graph distances between the remaining nodes in $H_{i_k}$ can only have decreased in comparison to their original graph distance in $G$. We therefore maintain the property that, for every node $u \in U_{i_{k+1}}$, for each representative point in $V_{i_{k+1}}$ within $u$, the points in $V_{i_k}$ that it represents can be at most $c$ times the diameter of $u$ apart in $H_{i_k}$. 
\end{proof}
\end{toappendix}

\begin{restatable}{lemma}{nodespercell}
    \label{lem:number_nodes_per_cell}
    For every node $u \in Q$, 
    the number of nodes added to $T$ is at most $O(c)$\lnote{$O(c\sqrt{d})$}. \lnote{Change this lemma to just talk about number connected components since primary purpose now size wspd first.}
\end{restatable}
\begin{toappendix}
\subsection{Proof of Lemma~\ref{lem:number_nodes_per_cell}}
\label{sec:nodespercell}
\nodespercell*
\begin{proof}
    From Lemma~\ref{lem:rep_c_connect} we know that each node in $V_{i_l}(s(u))$ must represent a valid $c$-connected set in $H_{i_{l-1}}(s(u))$. We now observe that one can upper bound the number of $c$-connected sets in $H_{i_{l-1}}(s(u))$ by the number of $c$-connected sets in $G(s(u))$. This observation follows from the fact that for any $1 \leq j \leq \ell$, $H_{i_j}$ was constructed by merging $c$-connected sets (w.r.t. diameter $\sqrt{d}2^{-i_j}$) in $H_{i_{j-1}}$, for every $u \in U_{i_j}$. Note that the argument used in the proof of Lemma~\ref{lem:rep_c_connect} shows that this process, for every $j$, can only cause the length of the paths between surviving nodes to become smaller. Since the position of surviving nodes does not change from their original position in $G$, it follows that the number of $c$-connected components in $H_{i_j}$ within $s(u)$ can only be smaller than that in $G$ within $s(u)$.  
    Since $G$ is $c$-packed, we can use the same argument as used in Lemma~\ref{lem:bounding_m_c-packed} to show that there can be at most $O(c)$ $c$-connected sets found by the algorithm. 
\end{proof}
\end{toappendix}

With the help of the above lemmas we are now ready to analyse the size of the resulting $W_G$ using a simple charging argument inspired by the one used in~\cite{book-geometric-apprx-algo-Peled2011}. 
\begin{lemma}
    \label{lem:size_and_separation_WSPDG}
    The resulting WSPD$_G$, $W$, is $\sigma$-well separated and is of size $O(c^3 \sigma n)$.
\end{lemma}
\begin{proof}
    The fact that $W$ is $\sigma$-well separated follows from the fact that we use the Euclidean distance as a lower bound on the distance between the two representatives, and we use upper bound on the graph diameter computed in Section~\ref{subsec:upperbounddiam} to upper bound the graph diameter, to determine whether a pair is $\sigma$-well separated.
    
    To prove the size of $W$ we use a simple charging argument. For a pair $(u,v) \in W$, let $\pi(v)$ denote the parent of $v$ in $T$. Assume the last call to the algorithm\lnote{reference the specific algorithm by Har-Peled from geom approx algos book and mention in construction that this is the algorithm used.} was via $(\pi(v), u)$. We charge the pair to $u$ and argue any node can be charged at most $O(c^2 \sigma)$ times. Since the pair $(\pi(v), u)$ was considered not well-separated by the algorithm, it follows that:
    \begin{align*}
        d(\pi(v), u) \leq d_G(\pi(v), u) < \gdub{\pi(v)}\sigma.
    \end{align*}
    Consider a geometric ball $B(u, r)$ of radius $r = (1+\sigma)\gdub{\pi(v)}$ centered at $u$. Note that connected component in $G$ represented by $\pi(v)$ must be fully contained inside $B$. By $c$-packedness, there can be at most $c\sigma +1$ candidates for $\pi(v)$. Since $\pi(v)$ can have at most $2^d \cdot O(c)$ children, it follows that there are $O(c^2 \sigma)$ candidates for $v$. We conclude a node $u$ can be charged at most $O(c^2\sigma)$ in this way. By Lemma~\ref{lem:number_nodes_per_cell} there are $O(c n)$ nodes in $T$. This concludes the lemma.
\end{proof}
